Multiplayer Performative Prediction: Learning in Decision-Dependent Games

Learning problems commonly exhibit an interesting feedback mechanism wherein the population data reacts to competing decision makers' actions. This paper formulates a new game theoretic framework for this phenomenon, called "multi-player performative prediction". We focus on two distinct solution concepts, namely (i) performatively stable equilibria and (ii) Nash equilibria of the game. The latter equilibria are arguably more informative, but can be found efficiently only when the game is monotone. We show that under mild assumptions, the performatively stable equilibria can be found efficiently by a variety of algorithms, including repeated retraining and the repeated (stochastic) gradient method. We then establish transparent sufficient conditions for strong monotonicity of the game and use them to develop algorithms for finding Nash equilibria. We investigate derivative free methods and adaptive gradient algorithms wherein each player alternates between learning a parametric description of their distribution and gradient steps on the empirical risk. Synthetic and semi-synthetic numerical experiments illustrate the results.

==> commands.tex <==




==> convexity.tex <==

In this section, we provide conditions under which the decision-dependent game is convex and strongly monotone, as defined below.

\begin{definition}[Convexity/strong monotonicity]\label{def:convexcontinuous}
The $N$--player game $\GN$ defined on a convex compact space $\Theta$ with $\mc{R}_i\in C^1(\Theta,\mb{R})$ is said to be a {convex continuous game} if, for all $i\in[N]$, the performative risk $\mc{R}_i(\cdot,\theta_{-i})$ is convex for every fixed $\theta_{-i}\in \Theta_{-i}$. Moreover, $\mc{G}_N$ is $\alpha$--strongly monotone if there exists an $\alpha>0$ such that
\begin{equation*}
    \la g(\theta')-g(\theta),\theta'-\theta\ra\geq \alpha\|\theta'-\theta\|^2, \ \ \forall \theta,\theta'\in \Theta.
\end{equation*}
\end{definition}
Strong monotonicity implies strict monotonicity---i.e., $\la g(\theta')-g(\theta),\theta'-\theta\ra>0$---which is equivalent to \emph{diagonal strict convexity}, the condition under which \cite{rosen1965existence} showed uniqueness of a Nash equilibrium in a general convex, continuous game. In particular, the following is a direct consequence.
 \begin{corollary}
    A convex $N$--player game $\GN$ admits a Nash equilibrium. If the game is additionally strictly monotone, then the Nash equilibrium is unique. 
\end{corollary}
For games with $\mc{R}_i\in C^2(\Theta,\mb{R})$, 
 $\alpha$--strong monotonicity is equivalent to the inequality $v^\top \nabla g(\theta)v \geq \alpha \|v\|^2$  holding for all vectors $v\in \mb{R}^d$ and for each $\theta\in \Theta$, and is equivalent to $\frac{1}{2}(\nabla g(\theta)+\nabla g (\theta)^\top)\succeq \alpha I$ for all $\theta$.
 

The following assumption
states that for each player $i\in [N]$, the distribution-loss pair 
 $(\Dzj,\lj)$ satisfies \emph{mixture dominance}, and is used to develop conditions under which the game $\GN$ is convex. 
 This assumption is also employed to show convexity 
 in the single player case 
 \citep{miller2021outside}.
 \begin{assumption}[Mixture Dominance]\label{ass:cvx}\label{a:mixturedominance}
For each player $i \in [N]$, for any $\theta\in \Theta$ and $\alpha\in [0,1]$, it holds:
 \begin{equation*}
     \E_{z_i\sim \mc{P}_1} [\lj(z_{i},\theta_i)]\leq \E_{z_i\sim \mc{P}_2}[\lj(z_{i},\theta_i)],\ 
\forall \theta_i',\theta_i''\in \Theta_i, 
 \end{equation*}
 where $\mc{P}_1=\Dzj(\alpha \theta_i'+(1-\alpha)\theta_i'',\theta_{-i}))$ and $\mc{P}_2=\alpha\mc{D}_i(\theta_i',\theta_{-i})+(1-\alpha)\mc{D}_i(\theta_i'',\theta_{-i})$.
\end{assumption}


As shown in Proposition A.4 of \cite{miller2021outside}, location-scale distributions satisfy Assumption~\ref{ass:cvx} when paired with any convex loss. 
For a game to be convex, it is sufficient to show that
each player's cost is convex in their choice variable holding all other players'
choice variables fixed.
The following result provides a sufficient condition on player costs $\mc{R}_i$ such that the game $\GN$ is convex. 
\begin{restatable}[Convexity]{proposition}{propconvexity}
\label{thm:cvx}
Consider an $N$--player game $\GN$  satisfying Assumptions~\ref{assump:convex}, \ref{ass:sensitive}, and \ref{ass:cvx}.
If $\xij\geq 2\betaj\epsj$ holds for each $i\in [N]$, then $\GN$ is a convex continuous game, and therefore admits a Nash equilibrium. 
\end{restatable}
Convexity for the single player setting was characterized in
\cite{miller2021outside};  the condition for convexity of each player's cost in
their own choice variable is equivalent to the single player setting, however,
we give an alternative proof approach which also gives insight into showing
strong monotonicity. 

The following assumption is analogous to the mixture dominance assumption which
enables the proof of convexity to go through.
\begin{assumption}
   For any $\theta\in \Theta$, the mapping \[u\mapsto \left(\frac{d}{du_1}\E_{z_1\sim
        \mc{D}_1(u_1,\theta_{-1})}\ell_1(z_1,\theta_1),\ldots,\frac{d}{du_N}\E_{z_N\sim
        \mc{D}_N(u_N,\theta_{-N})}\ell_N(z_N,\theta_N)\right) \] is monotone.
     \label{a:monotone}
     \ljr{check this is even right}
 \end{assumption}
\begin{restatable}[Strong Monotonicity]{proposition}{propmonotone}
Consider a  two-player game $\Gn{N}=(\mc{R}_1,\ldots, \mc{R}_N)$
defined by  $\mc{R}_i\in C^2(\Theta,\mb{R})$ for each $i\in[N]$, and such that
Assumptions~\ref{assump:convex}, \ref{ass:sensitive}, \ref{ass:cvx}, and \ref{a:monotone} hold.    
Define the parameter
\[\alpha:= \min_{i\in [N]}~\{\xi_i-\beta_i\varepsilon_i\}.\]
Then, in the regime
$\alpha>0$,
the game is $\alpha$-strongly monotone.
\label{prop:2player_strongmonotone}
\end{restatable}

\textbf{Structural Stability of Nash Equilibrium.} 
In Section~\ref{sec:algs}, we study gradient-based learning in stochastic games---that is, players seek equilibrium through a t\^atonnement process by which they follow an estimate of their gradient rather than the true gradient.
 The game defined by empirical estimates of the risk can be viewed as a 
 `perturbation' of the game $\mc{G}_N$.
It is important to understand the closeness (by way of a structural stability analysis) of the equilibria of the perturbed game to that of the original game.
 In Appendix~\ref{app:risk_games}, we show  that strong monotonicity is a structurally stable property of the multiplayer performative prediction games we study in this paper.  
 
 Moreover, under Assumption~\ref{assump:locationscale}, we give a bound on the distance between the Nash equilibrium $\theta^\ast$ of
 $\GN$ and the Nash equilibrium $\hat{\theta}^{(n)}$ of the game defined by the estimated empirical risks $\widehat{\mc{R}}_i^{(n)}=\frac{1}{n}\sum_{i=1}^n\ell_i(z_i,\theta_i)$ with $z_i\sim \widehat{\mc{D}}_i(\theta_i,\theta_{-i})$, where $\widehat{\mc{D}}_i(\theta_i,\theta_{-i})$ is the location scale distribution defined by 
 \[z_i\sim \widehat{\mc{D}}_i(\theta_i,\theta_{-i}) \ \Longleftrightarrow\ z_i=q_i+\widehat{\mu}_i\theta_i+\widehat{\gamma}_i\theta_{-i}.\]
 In particular, suppose players use an estimator for $\widehat{p}_i=(\widehat{\mu}_i,\widehat{\gamma}_i)$ satisfying the following: for any $n\geq \Omega(d+m+\log(N/\delta)$, with with probability $1-\delta$, the estimate $\|\widehat{p}_i-p_i\|=\mc{O}((\frac{d+m+\log(N/\delta)}{n})^{1/2})$  holds. In this setting, we show that 
 with probability $1-3N\delta$, the estimate 
 $\|\hat{\theta}^{(n)}-\theta^\ast\|=\mc{O}((\log(1/\delta)\frac{d\log n}{n})^{1/2}+(\frac{d+m+\log(N/\delta)}{n})^{1/2})$ holds.

 




